A Deep Cybersickness Predictor through Kinematic Data with Encoded Physiological Representation

Users would experience individually different sickness symptoms during or after navigating through an immersive virtual environment, generally known as cybersickness. Previous studies have predicted the severity of cybersickness based on physiological and/or kinematic data. However, compared with kinematic data, physiological data rely heavily on biosensors during the collection, which is inconvenient and limited to a few affordable VR devices. In this work, we proposed a deep neural network to predict cybersickness through kinematic data. We introduced the encoded physiological representation to characterize the individual susceptibility; therefore, the predictor could predict cybersickness only based on a user's kinematic data without counting on biosensors. Fifty-three participants were recruited to attend the user study to collect multimodal data, including kinematic data (navigation speed, head tracking), physiological signals (e.g., electrodermal activity, heart rate), and Simulator Sickness Questionnaire (SSQ). The predictor achieved an accuracy of 97.8\% for cybersickness prediction by involving the pre-computed physiological representation to characterize individual differences, providing much convenience for the current cybersickness measurement.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by $Author: jpeltier $ $Date: 2007-04-03 16:51:34 -0700 (Tue, 03 Apr 2007) $
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers
according to the specifications for submission to conferences sponsored
by the IEEE Visualization & Graphics Technical Committee (VGTC). This
includes:

Conferences that use the 'conf' document option:
- IEEE Virtual Reality
- IEEE Symposium on 3D User Interfaces
- Symposium on Haptic Interfaces for Virtual Environment and Teleoperator Systems
- IEEE Symposium on Asia Pacific Visualisation
- IEEE Symposium on Interactive Ray Tracing
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Symposium on Visual Analytics Science and Technology
- IEEE Visualization Conference (Posters Only)
- IEEE Information Visualization Conference (Posters Only)
- IEEE Symposium on Volume Graphics

It contains 11 files/directories:

README          - this file
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default conference mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> ppt/metadata <==
	
256p1	
257p2	
258p3	
259p4	
260p5	
261p6	
262p7	
263p8	
264p9

265p10

266p11

267p12

268p13

269p14

270p15"

2147483648p16*

2147483649p17*

2147483650p18*

2147483651p19*

2147483652p202E
n	
3n_i2	
4n_i3	
5n_i4	
6n_i5	
7n_i6	
8n_i72!
p16
10p16_i2
11p16_i32!
p17
13p17_i2
14p17_i32!
p18
16p18_i2
17p18_i32$
p1:notes
21p1_g1
22p1_g22œ
p1i
24p1_i22\
0W
U{"type":"shape","subtype":"text","uid":1696310178700,"page":"p1","targets":["p1_i2"]}
25p1_i7
26p1_i1026
27p1_i10302$
p2:notes
29p2_g3
30p2_g42»
p2
32p2_i2
33p2_i3
34p2_i6
35p2_i7
36p2_i12
37p2_i8
38p2_i11
39p2_i15
40p2_i13
41p2_i14
42g24ae1c02e8e_0_2
43g24ae1c02e8e_0_42$
p3:notes
45p3_g5
46p3_g62ª

p3
48p3_i2Õ	
49p3_i32\
1W
U{"type":"shape","subtype":"text","uid":1696310329131,"page":"p3","targets":["p3_i3"]}2\
2W
U{"type":"shape","subtype":"text","uid":1696310329131,"page":"p3","targets":["p3_i3"]}2\
3W
U{"type":"shape","subtype":"text","uid":1696310329131,"page":"p3","targets":["p3_i3"]}2\
4W
U{"type":"shape","subtype":"text","uid":1696310329131,"page":"p3","targets":["p3_i3"]}2\
5W
U{"type":"shape","subtype":"text","uid":1696310329131,"page":"p3","targets":["p3_i3"]}2\
6W
U{"type":"shape","subtype":"text","uid":1696310329131,"page":"p3","targets":["p3_i3"]}2\
7W
U{"type":"shape","subtype":"text","uid":1696310329131,"page":"p3","targets":["p3_i3"]}2\
8W
U{"type":"shape","subtype":"text","uid":1696310329131,"page":"p3","targets":["p3_i3"]}2\
9W
U{"type":"shape","subtype":"text","uid":1696310329131,"page":"p3","targets":["p3_i3"]}2]
10W
U{"type":"shape","subtype":"text","uid":1696310329131,"page":"p3","targets":["p3_i3"]}2]
11W
U{"type":"shape","subtype":"text","uid":1696310329131,"page":"p3","targets":["p3_i3"]}2]
12W
U{"type":"shape","subtype":"text","uid":1696310329131,"page":"p3","targets":["p3_i3"]}2]
13W
U{"type":"shape","subtype":"text","uid":1696310329131,"page":"p3","targets":["p3_i3"]}
50p3_i4
51p3_i5
52p3_i7
53p3_i8
54p3_i92$
p4:notes
56p4_g7
57p4_g82
p4
59p4_i2
60p4_i52%
p5:notes
62p5_g9
63p5_g102o
p5
65p5_i2
66p5_i9
67p5_i11
68p5_i12
69p5_i15
70p5_i17
71g24ae1c02e8e_0_102&
p6:notes
73p6_g11
74p6_g122º
p6
76p6_i2
77p6_i8
78p6_i15
79p6_i20
80p6_i21
81p6_i23
82p6_i24
83p6_i26
84g24ae1c02e8e_0_5
85g24ae1c02e8e_0_7
86g24ae1c02e8e_0_82&
p7:notes
88p7_g13
89p7_g142,
p7
91p7_i2
92p7_i8
93p7_i102&
p8:notes
95p8_g15
96p8_g162,
p8
98p8_i2
99p8_i3
100p8_i42(
p9:notes
102p9_g17
103p9_g182.
p9
105p9_i2
106p9_i4
107p9_i52+
	p10:notes
109p10_g19
110p10_g202â
p10
112p10_i2
113p10_i7
114p10_i24
115p10_i8
116p10_i14
117p10_i15
118p10_i16
119p10_i17
120p10_i18
121p10_i19
122p10_i20
123p10_i22
124p10_i26
125p10_i272+
	p11:notes
127p11_g21
128p11_g222ê
p11
130p11_i2
131p11_i3
132p11_i22
133p11_i12
134p11_i6
135p11_i9
136p11_i10
137p11_i11
138p11_i13
139p11_i21
140p11_i24
141p11_i25
142p11_i27
143g24ae1c02e8e_0_02+
	p12:notes
145p12_g23
146p12_g242Ò
p12
148p12_i6
149p12_i8
150p12_i9
151p12_i11
152p12_i12
153p12_i13
154p12_i14
155p12_i15
156p12_i16
157p12_i18
158p12_i19
159p12_i20
160p12_i212+
	p13:notes
162p13_g25
163p13_g262#
p13
165p13_i2
166p13_i42+
	p14:notes
168p14_g27
169p14_g282
p14
171p14_i22+
	p15:notes
173p15_g29
174p15_g30:ß
AAAA5Mc5Sn4Ÿ
AAAA5Mc5Sn4AAAA5Mc5Sn4(
	text/html题目的字体大小统一")

text/plain题目的字体大小统一*…
Yuyang WangY//lh3.googleusercontent.com/a/ACg8ocJapyDh3vhvcxStifa0CZiW-Iim06GSHh4HzZN7m4T_=s50-c-k-no"105065547256403755187(8H0§êݟ¯18§êݟ¯1Jr

text/plaindA Deep Cybersickness Predictor through Kinematic Data with Encoded Physiological RepresentationZ90qryrw8aflrl
Yuyang Wang[
Y//lh3.googleusercontent.com/a/ACg8ocJapyDh3vhvcxStifa0CZiW-Iim06GSHh4HzZN7m4T_=s50-c-k-no xšª题目的字体大小统一§êݟ¯1 §êݟ¯1*I
!14e6Zj9d_Hu1DEXfaFerzzxnLzq0ekDBb$

text/plainISMAR23_ruichenli.pptxBU{"type":"shape","subtype":"text","uid":1696310178700,"page":"p1","targets":["p1_i2"]}:Â
AAAA5Mc5Sn8'
AAAA5Mc5Sn8AAAA5Mc5Sn8=
	text/html0不同层级的大纲符号,要保持不同。">

text/plain0不同层级的大纲符号,要保持不同。*…
Yuyang WangY//lh3.googleusercontent.com/a/ACg8ocJapyDh3vhvcxStifa0CZiW-Iim06GSHh4HzZN7m4T_=s50-c-k-no"105065547256403755187(8H0÷‰çŸ¯18÷‰çŸ¯1J"

text/plain…CS prediction using data from integrated sensors in HMDs 
	These data struggle to reflect individual differences. 
CS prediction using physiological data and biometrics
Requires external biosensors;
Requires users to limit their interaction experience.Ze3jkf7bc6vtwrl
Yuyang Wang[
Y//lh3.googleusercontent.com/a/ACg8ocJapyDh3vhvcxStifa0CZiW-Iim06GSHh4HzZN7m4T_=s50-c-k-no xšª20不同层级的大纲符号,要保持不同。÷‰çŸ¯1 ÷‰çŸ¯1*I
!14e6Zj9d_Hu1DEXfaFerzzxnLzq0ekDBb$

text/plainISMAR23_ruichenli.pptxBU{"type":"shape","subtype":"text","uid":1696310329131,"page":"p3","targets":["p3_i3"]}B
en-USJ!14e6Zj9d_Hu1DEXfaFerzzxnLzq0ekDBb
